LEGO-Prover: Neural Theorem Proving with Growing Libraries

Despite the success of large language models (LLMs), the task of theorem proving still remains one of the hardest reasoning tasks that is far from being fully solved. Prior methods using language models have demonstrated promising results, but they still struggle to prove even middle school level theorems. One common limitation of these methods is that they assume a fixed theorem library during the whole theorem proving process. However, as we all know, creating new useful theorems or even new theories is not only helpful but crucial and necessary for advancing mathematics and proving harder and deeper results. In this work, we present LEGO-Prover, which employs a growing skill library containing verified lemmas as skills to augment the capability of LLMs used in theorem proving. By constructing the proof modularly, LEGO-Prover enables LLMs to utilize existing skills retrieved from the library and to create new skills during the proving process. These skills are further evolved (by prompting an LLM) to enrich the library on another scale. Modular and reusable skills are constantly added to the library to enable tackling increasingly intricate mathematical problems. Moreover, the learned library further bridges the gap between human proofs and formal proofs by making it easier to impute missing steps. LEGO-Prover advances the state-of-the-art pass rate on miniF2F-valid (48.0% to 57.0%) and miniF2F-test (45.5% to 47.1%). During the proving process, LEGO-Prover also manages to generate over 20,000 skills (theorems/lemmas) and adds them to the growing library. Our ablation study indicates that these newly added skills are indeed helpful for proving theorems, resulting in an improvement from a success rate of 47.1% to 50.4%. We also release our code and all the generated skills.

==> docs/introduction.tex <==

\section{Introduction}
\begin{figure}[t!]
   \centering
   \includegraphics[width=\textwidth]{imgs/illustrate.pdf}
  \caption{Overview of LEGO-Prover. The algorithm consists of 2 parts: Formalizer and Evolver. \xd{add more captions to explain}}
  \label{fig:idea}
% \vspace{3mm}
\end{figure}

\xd{add reference in intro}

% As an example of complex reasoning involving rigorous logical inference and abstract concepts, m
The ability of mathematical reasoning is considered an important aspect for benchmarking the performance of large language models (LLMs)~\citep{touvron_llama_2023,touvron_llama2_2023, yu2023metamath,luo_wizardmath_2023}. Despite the remarkable successes that LLMs have achieved in numerous language reasoning problems, there are still significant shortcomings in the realm of mathematical reasoning. Current research on the application of large language models to mathematical reasoning primarily focuses on math word problems, as in these problems, the correctness of mathematical reasoning can be reliably measured by matching answers. It is well-known that theorem proving is more challenging to assess than mathematical calculations, but formal mathematical systems provide precise, usable, and scalable evaluation criteria for this purpose. In formal mathematical systems, theorems expressed in natural language are translated into formal code and then verified the correctness of their proofs using a formal verifier, and in this way organizes all mathematical propositions into a searchable and easily modifiable unified library.

% Large language models (LLMs) offer a promising solution to tackle the alignment problem. LLMs have demonstrated remarkable reasoning capabilities comparable to human intelligence in many tasks, equipped with a substantial number of learnable parameters and trained on extensive text data. In addition to advancements in fine-tuning techniques, current research has also focused on utilizing and developing external tools to unlock the potential for enhancing LLMs. This approach aligns well with the classical idea of formal mathematics, which employs verifiers to verify the correctness of theorem proofs.

% Furthermore, some researchers have devised techniques to create reusable commands, known as skills, for LLM agents. These skills are then combined in a combinatorial manner to construct new skills. This approach aligns perfectly with the cumulative nature of mathematical theories, particularly in formalized mathematics. Formalized mathematics overcomes the ambiguity and lack of rigidity found in natural languages by rigorously and clearly describing references to existing theorems in the code of formal mathematics. In this setting, the usefulness of lemma accumulation for theorem proving can be rigorously and completely portrayed.



% Despite the success of large language models (LLMs), the task of theorem proving still remains one of the few hardest reasoning tasks that are far from being fully solved by them. Prior methods using language models have demonstrated promising results but they still struggle to even prove middle school level theorems. One common limitation of these methods is that they assume a \emph{fixed} theorem library during the whole theorem proving process. But as we all know, creating new useful theorems or even new theories is not only helpful but crucial and necessary for advancing mathematics and prove harder and deeper results.
% In this work, we present \textit{LEGO-Prover}, a new framework that employs a growing theorem/skill library to augment the capability of LLMs used in theorem proving. New theorems are created by coming up with lemmas relevant to a given theorem by prompting an LLM. These lemmas are further evolved (also by prompting an LLM) to enrich the library to another scale.
% Modular and reusable lemmas are constantly added to the library to enable tackling increasingly intricate mathematical problems. Moreover, the learned  library further bridges the gap between human-generated mathematical proofs and formal proving languages, enhancing the current formal theorem library. 
% LEGO-Prover obtains state-of-the-art pass rates on miniF2F-valid ($48.0\% \to 57.0\%$) and miniF2F-test ($X\% \to Y\%$). During the proving process, LEGO-Prover also manages to generated over $XXX$ theorems and add them to the growing library. An ablation study indicates that these newly added theorems are indeed helpful for proving theorems, with an improvement from $47.1\% \to 50.4\%$. We also 

% It is widely acknowledged that the progress of mathematics relies on the consensus among experts, and mathematical discoveries are closely tied to human cognitive processes. However, traditional mathematical work heavily depends on manually verifying proofs, which poses challenges to the rigor of mathematical proofs and the efficiency of communication within the mathematical community. To address these challenges, formalized mathematics advocates for reconstructing existing mathematics using formal languages \citep{avigad2023formal}. It 

% Employing formal verifiers to validate the correctness of mathematical proofs and organizes all mathematical propositions into a searchable and easily modifiable unified codebase, 

In recent years, the formalized mathematics community has made significant progress in programming languages, verification systems, and automated theorem-proving tools \citep{gpt-f,dsp}. For example, \citet{gpt-f} use large language models to generate proof step candidate and perform search algorithms to conduct the whole proof.
\citet{dsp} take a step forward and attempt to formalize the complete proof in a 3 step manner: Draft, Sketch, and Prove.
However, most existing works can be classified into plain prover, which generates proof step directly without any external components (e.g., memory).

% formalized mathematics still faces numerous challenges and cannot yet meet the practical requirements of working mathematicians. Mathematicians often struggle to align their own understanding of specific concepts with the formal definitions in the mathematical library. This alignment process involves tedious translation and equivalence proofs, which can be time-consuming and hinder the progress of mathematical reasoning tasks. 



To solve the shortcomings of plain prover, inspired by these insights and the modularity of LEGO building blocks, we present \textit{LEGO-Prover}, a novel approach designed to address theorem proving problems of increasing difficulty by dynamically generating lemmas. As illustrated in Figure~\ref{fig:idea}, when the process of theorem proving unfolds, the generated lemmas are accumulated into a growing skill library. These lemmas are then refined using conceptual patterns and subsequently reused in future theorem proving problems. This iterative process allows us to construct more complex and powerful skills by utilizing the gathered skills, which are combined into skill libraries with combinational referential relations. 

% This is made possible through the use of a growing skill library, which serves as a repository of reusable mathematical reasoning units. Specifically, LEGO-Fomalizer is composed of two major components.

% The first is the \textit{Formalizer}, which actively retrieves reusable skills (lemma blocks) from a growing skill library to assist the LLM in formalizing new mathematical problems. Upon successful formalization, the \textit{Formalizer} concludes the reusable and useful lemma as skills and adds to the skill library.
% The second key component is the \textit{Skill Evolver}, which iteratively refines and evolves the skills stored in the library. It takes existing skills as input, identifies potential problems that can be solved using these skills, and then employs a diverse set of evolving directions to refine them. Verified skills that have evolved successfully are incorporated back into the skill library, further enhancing its capabilities for future tasks.
% This dual-component architecture not only allows for the reuse of formalized skills but also ensures their continuous evolution, making the \textit{LEGO-Prover} a dynamic and adaptive system capable of composing complex proof.

We conducted extensive experiments on the popular theorem-proving dataset miniF2F to validate the effectiveness of our proposed approach. Our LEGO-Prover significantly outperforms competing approaches, achieving a pass rate of -\% on the miniF2F test dataset, a -\% absolute improvement over the previous state-of-the-art methods. Beyond this, our case study reveals that LLMs formalize problems modularly akin to LEGO block assembly, further corroborating our methodology's effectiveness. Finally, the learned skill library also serves as a valuable enhancement to the standard Isabelle library, which includes many useful high-level lemmas broadly applicable to various problems.

To summarize, the key contributions of this paper are as follows:
\begin{itemize}
    \item 
    \item 
    \item 
\end{itemize}

% The automation of formal reasoning tasks, such as theorem proving and mathematical proof formalization, represents a formidable challenge and an active area of research within the domain of artificial intelligence \citep{gpt-f,pact,jiang2022thor,wholeproof,BansalLRSW19,lample_hypertree_2022,dsp,jianglisa,zhao2023decomposing,yang2023leandojo,wang2023dt,liu2023fimo}. The formalization of mathematical proof typically relied on human experts to transcribe and translate intricate mathematical concepts into structured formal languages verifiable by interactive theorem prover like Lean \citep{de_moura_lean_2015}, Isabelle \citep{paulson_isabelle_1994}, Metamath \citep{megill_metamath_2019}. This process, while robust, is often labor-intensive and demands a high level of expertise. 

% Large language models (LLMs) emerged as a promising avenue, with their capacity to process and produce human-like text, opening the door to the idea of automated mathematical proof formalization. \xd{too long, try to move some into related work}\cite{wu2022autoformalization} study the possibility of formalizing the natural language theorem statements into formal statements written in Isabelle. \cite{dsp} takes a step forward and tries to formalize the complete proof in a 3 step manner. The draft step generates the natural language proof using the natural language problem statement (could be replaced with actual human written proof). The sketch step utilizes the natural language proof to guide the LLM to generate proof sketches in Isabelle, which states the primary proof steps/conjectures in the proof. The final proof step completes the proof by using Isabelle's built-in rule-based ATPs (also known as the sledgehammer) like Z3 \citep{demoura2008z3}, CVC4 \citep{barrett2011cvc4},
% SPASS \citep{weidenbach2009spass}, Vampire \citep{riazanov2002design}, E \citep{jakubuuv2016extending}. \citep{zhao2023decomposing} is the follow-up work for DSP, this approach uses cross-verified step-by-step natural language proof that better guides the LLM to generate the sketch. Additional example re-ordering method also helps improve the performance of auto-formalization. 

% Despite their promising results, these methods encounter significant bottlenecks. Specifically, these techniques are limited by the inherent shortcomings of static LLM, which are unable to adapt or extend their formalization capabilities to address increasingly complex and challenging problems without fine-tuning. A fundamental obstacle to automated formalization lies in the gap between natural language proofs and formal theorem representations. As illustrated in Figure \ref{fig:main_dts}\xd{should be figure 1?}, while simple proof tactics may be intuitively straightforward for humans, they can become inordinately verbose and complex when rendered in formal language. Even though large language models like GPT-3.5 or GPT-4 \citep{gpt4} are capable of generating these ostensibly trivial proofs with a relatively high degree of accuracy, their effectiveness sharply declines when it comes to composing complex proofs that involve multiple simple operations. 




% Specifically, LEGO-Fomalizer is composed of two major components: 1) When formalizing a new problem, the formalizer retrieves useful skill (lemma blocks) from skill library. and ask the LLM to foramlize the problem with the help of the retrived skills given. When a problem is successfully formalized, the formalizer conlude the useful reusable lemma as skills and add to the skill library. 2) the second part is the skill evolver, the skill evolver will continuously evolve the skill in the skill library. For each evolve, The evolver takes a skill in the skill library as input, and retrieve a set of possible problem to solve. We ask the large languge model to evolve the skill by trying to make the skill more helpful for solving the problem. The evolver will randomly select its evolving direction among 7 specific evolving directions like altering conditions, broadening definitions, parameterizing, and switching domains. and 3 general evolve direction that generally evolve the skill, critique and evolve the skill, or take in multiple skills and try to compose these skills. The evolved skill that passes the verification of the Isabelle theorem prover will be added to the skill library, waiting for Formalizer to retrived or evlove further by the evolver.



% Our contributions are listed as follows:
% \begin{itemize}
%    \item We proposed LEGO-Prover, a novel method for auto-formalization, which utilizes a growing skill library to construct proof in a modularity way.
%    \item The learned skill library serves as a valuable enhancement on the standard Isabelle library, which includes many useful high-level lemmas that are useful for other problems. 
%    \item Our LEGO-Prover substantially improved upon state-of-the-art approaches b.
% \end{itemize}
